Inducing Cooperative behaviour in Sequential-Social dilemmas through Multi-Agent Reinforcement Learning using Status-Quo Loss

In social dilemma situations, individual rationality leads to sub-optimal group outcomes. Several human engagements can be modeled as a sequential (multi-step) social dilemmas. However, in contrast to humans, Deep Reinforcement Learning agents trained to optimize individual rewards in sequential social dilemmas converge to selfish, mutually harmful behavior. We introduce a status-quo loss (SQLoss) that encourages an agent to stick to the status quo, rather than repeatedly changing its policy. We show how agents trained with SQLoss evolve cooperative behavior in several social dilemma matrix games. To work with social dilemma games that have visual input, we propose GameDistill. GameDistill uses self-supervision and clustering to automatically extract cooperative and selfish policies from a social dilemma game. We combine GameDistill and SQLoss to show how agents evolve socially desirable cooperative behavior in the Coin Game.

==> Multi-Agent ICLR -- arxiv - updated/analysis.tex <==



==> Multi-Agent ICLR -- arxiv - updated/approach.tex <==
\section{Approach}
\label{sec:approach}


%\begin{figure*}
%    \includegraphics[width=\linewidth]{images/skill_detection_network.png}
%    \caption{Network architecture diagram for skill discovery network}
%    \label{fig:skill_detection_network}
%\end{figure*}

%\begin{figure}
%    \includegraphics[width=\linewidth]{images/action_prediction_network.png}
%    \caption{Neural Network architecture for the Action Prediction Network}
%    \label{fig:action_prediction_network}
%\end{figure}


\subsection{Social Dilemmas modeled as Iterated Matrix Games}
We adopt the definitions in \citet{foerster2018learning}.
We model social dilemmas as general-sum Markov (simultaneous move) games.
A multi-agent Markov game is specified by $G = \langle$$S$, $A$, $U$, $P$, $r$, $n$, $\gamma$$\rangle$.
$S$ denotes the state space of the game. 
$n$ denotes the number of agents playing the game.
At each step of the game, each agent $a \in A$, selects an action $u^a \in U$.
$\Vec{u}$ denotes the joint action vector that represents the simultaneous actions of all agents. 
The joint action $\Vec{u}$ changes the state of the game from $s$ to $s'$ according to the state transition function $P(s'|\Vec{u},s): S \times \textbf{U} \times S \rightarrow  [0, 1]$.
At the end of each step, each agent $a$ gets a reward according to the reward function $r^{a}(s, \Vec{u}): S \times \textbf{U} \rightarrow \mathbb{R}$. 
The reward obtained by an agent at each step is a function of the actions played by all agents. 
For an agent, $a$, the discounted future return from time $t$ is defined as $R_{t}^{a} = \sum_{l=0}^{\infty} \gamma^{l} r_{t+l}^{a}$,
where $\gamma \in [0, 1)$ is the discount factor.
Each agent independently attempts to maximize its expected total discounted reward. 

Matrix games are the special case of two-player perfectly observable Markov games~\cite{foerster2018learning}. 
Table~\ref{tab:payoff_matrix} shows examples of matrix games that represent social dilemmas.
Consider the Prisoner's Dilemma matrix game in Table~\ref{tab:payoff_matrix_ipd}.
Each agent can either cooperate ($C$) or defect ($D$).
For an agent, playing $D$ is the rational choice, regardless of whether the other agent plays either $C$ or $D$.
Therefore, if both agents play rationally, they each receive a reward of $-2$. 
However, if each agent plays $C$, then it will obtain a reward of $-1$. 
This fact that individually rational behavior leads to a sub-optimal group (and individual) outcome highlights the dilemma. 

In Infinitely Iterated Matrix Games, agents repeatedly play a particular matrix game against each other. 
In each iteration of the game, each agent has access to the actions played by both agents in the previous iteration.
Therefore, the state input to an RL agent consists of the actions of both agents in the previous iteration of the game.
We adopt this state formulation to remain consistent with \citet{foerster2018learning}. 
The infinitely iterated variations of the matrix games in Table~\ref{tab:payoff_matrix} represent sequential social dilemmas. 
For ease of representation, we refer to infinitely iterated matrix games as iterated matrix games in subsequent sections. 

\subsection{Learning Policies in Iterated Matrix Games: The Selfish Learner}
\label{sec:approach:selfish-learner}

The standard method to model agents in iterated matrix games is to model each agent as a Deep RL agent that independently attempts to maximize its expected total discounted reward.
Several approaches to model agents in this way use policy gradient-based methods~\cite{sutton2000policy, williams1992simple}).
Policy gradient methods update an agent's policy, parameterized by $\theta^{a}$, by performing gradient ascent on the expected total discounted reward $\E [R_{0}^{a}]$. 
Formally, let $\theta^{a}$ denote the parameterized version of an agent's policy $\pi^{a}$ and $V_{\theta^{1},\theta^{2}}^{a}$ denote the total expected discounted reward for agent $a$. 
Here, $V^{a}$ is a function of the policy parameters $(\theta^{1}, \theta^{2})$ of both agents. 
In the $i^{th}$ iteration of the game, each agent updates $\theta_{i}^{a}$ to $\theta_{i+1}^{a}$, such that it maximizes it's total expected discounted reward. $\theta_{i+1}^{a}$ is computed as follows:
% \vspace{-6pt}
\begin{equation}
    \begin{split}
        \theta_{i+1}^{1} & = argmax_{\theta^{1}} V^{1}(\theta^{1}, \theta_{i}^{2})\\
        \theta_{i+1}^{2} & = argmax_{\theta^{2}} V^{2}(\theta_{i}^{1}, \theta^{2})\\
    \end{split}
\end{equation}
For agents trained using reinforcement learning, the gradient ascent rule to update $\theta_{i+1}^{1}$ is:
\begin{equation}
    \begin{split}
        f_{nl}^{1} & = \nabla_{\theta^{i}_{1}} V^{1} (\theta_{i}^{1}, \theta_{i}^{2}) \cdot \delta \\
        \theta_{i+1}^{1} & = \theta_{i}^{1} + f_{nl}^{1} (\theta_{i}^{1}, \theta_{i}^{2}) 
    \end{split}
    \label{eq:naive_learner_update_rule}
\end{equation}

where $\delta$ is the step size of the updates.
\todopb{they use policy-gradient and actor-critic -- add this information as well, now it does not have much information}

In the Iterated Prisoner's Dilemma (IPD) game, agents trained with the policy gradient update method converge to a sub-optimal mutual defection equilibrium (Figure~\ref{fig:results_IPD}, \cite{Peysakhovich1707.01068}).
This sub-optimal equilibrium attained by Selfish Learners motivates us to explore alternative methods that could lead to a desirable cooperative equilibrium.
We denote the agent trained using policy gradient updates as a Selfish Learner ($SL$). 


\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{images/rl_gameplay_summary_new.pdf}
    \caption{
    Intuition behind $SQLearner$.
    At each step, the $SQLoss$ encourages an agent to imagine the consequences of sticking to the status-quo by imagining an episode where the status-quo is repeated for $\kappa$ steps.  
    Section~\ref{sec:approach:SQLoss} describes $SQLoss$ in more detail. 
    }
    \label{fig:rl_imaginative_learning}
\end{figure}


\begin{comment}

The notation, (A, B) denotes the first agent takes an action \textit{A} and the second agent takes an action \textit{B}.
This equilibrium describes the scenario when both players always defect. 
According to the Folk theorem~\cite{folk_theorem,Fudenberg}, the IPD has infinitely many Nash equilibria, out of which $(D, D)$ is the most commonly occurring NE in deep reinforcement learning setup~\cite{foerster2018learning}.
From the reward matrix, it is clear that both players would do better if they played $(C, C)$. 
However, this is not a stable equilibrium because $a_1$ can improve its reward by playing $D$ instead of $C$ since $R_1(D, C) > R_1(C, C)$. 
Here, $R_1$ denotes the reward for $a_1$. 
The same reasoning holds for $a_2$. 
Therefore, both players have an incentive to switch from $(C, C)$ to $(D, D)$. 
In contrast, if the two players are playing $(D, D)$, then neither has an incentive to change their action. 
\end{comment}


% \theoremstyle{plain}

% \newtheorem{defn}[thm]{Definition} % definition numbers are dependent on theorem numbers
\begin{comment}

\begin{definition}
Iterative Prisoner's Dilemma (IPD). In the iterative prisoner's dilemma, players play several instances of the single-step prisoner's dilemma sequentially. At each iteration, players have access to the past actions taken by all players. 
\end{definition}
\end{comment}

\begin{comment}


When RL agents optimize for individual rewards in an IPD, they reach a state of mutual defection, as discussed earlier.
Here, we propose an approach to evolve cooperative behavior in two-player matrix games. 
Our approach has two components. 
\begin{itemize}
% \vspace{-3pt}
    \item In Section~\ref{sec:SQLoss}, we describe the Status-Quo loss ($SQLoss$). 
    We show how agents trained with an additional $SQLoss$ evolve cooperative behavior in a multi-agent game setting. 
    \item In Section~\ref{sec:GameDistill}, we describe the architecture of the \ipdistill component, which uses self-supervised skill discovery to transform a game with visual input into its IPD formulation.
\end{itemize}
We then show how applying \ipdistill along with $SQLoss$ evolves cooperative behavior between agents in the Coin game.  
\end{comment}

\begin{comment}

\subsection{Learning Policies in Iterated Matrix Games: The Selfish Learner in an $\eta$-stationary environment}
A Selfish Learner plays the iterated matrix game and performs updates defined by Equation~\ref{eq:naive_learner_update_rule}. 
One of the main reasons that a $SL$ agent learns to defect in a sequential social dilemma is that it does not always see the consequences of its selfish behavior. 
However, if the environment enforces a \textit{stationary policy}[???] for $\eta$ horizons, then both $SL$ agents are forced to stick with their action for $\eta$ steps.
Figure~\ref{fig:rl_imaginative_learning} shows the states, rewards, and actions for this situation.
A $SL$ agent in an $\eta$-stationary environment is incentivized to take actions that optimize long-term rewards while having a stationary policy.

Figure~\ref{fig:ipd_results_sticky=20} shows the level of cooperation of two $SL$ agents playing the iterated prisoner's dilemma in a 20-stationary environment. 
The stationary environment has two benefits.
First, it reduces the likelihood that an agent will defect in a mutually cooperative situation. 
This `cooperation stickiness' is because the short-term exploitative gain from switching actions is overcome by the long-term costs (because of stationarity) of mutual defection. Second, $SL$ agents in a stationary environment have more incentive to optimize long-term rewards rather than focus on the short-term gains of defection. 


However, in general, it might not be possible to alter environment dynamics to enforce stationarity.
Therefore, we introduce a Status-Quo loss that encourages a stationary policy and, subsequently, cooperative behavior. 
\end{comment}

\subsection{Learning Policies in Iterated Matrix Games: The Status-Quo Aware Learner ($SQLoss$)}
\label{sec:approach:SQLoss}

\subsubsection{$SQLoss$: Intuition}
Why do independent, selfish learners converge to mutually harmful behavior in the IPD?
To understand this, consider the payoff matrix for a single iteration of the IPD in Table~\ref{tab:payoff_matrix_ipd}.
In each iteration, an agent can play either $C$ or $D$.
Mutual defection $(D, D)$ is worse for each agent than mutual cooperation $(C, C)$.
However, one-sided exploitation $(D, C)$ is better than mutual cooperation for the exploiter and far worse for the exploited. 
Therefore, as long as an agent perceives the possibility of exploitation ($(D, C)$ or $(C, D)$), it is drawn to defect, both to maximize reward (through exploitation) and minimize loss (through being exploited). 
To increase the likelihood of cooperation, it is important to reduce instances of exploitation between agents. 
We posit that, if agents mostly only either mutually cooperate $(C, C)$ or mutually defect $(D, D)$, then they will learn to prefer $C$ and achieve a socially desirable cooperative equilibrium.   

Motivated by this idea, we introduce a status-quo loss ($SQLoss$) for each agent derived from the idea of imaginary game-play, as depicted in Figure~\ref{fig:rl_imaginative_learning}. 
Intuitively, the loss encourages an agent to imagine an episode where the status-quo (current situation) is repeated for a number of steps. 
This imagined episode causes the exploited agent (in $(D, C)$) to perceive a continued risk of exploitation and, therefore, quickly move to $(D, D)$.
Hence, for an agent, the short-term gain from exploitation $(D, C)$ is overcome by the long-term loss from mutual exploitation $(D, D)$. 
Therefore, agents move towards either mutual cooperation $(C, C)$ or mutual defection $(D, D)$.
With exploitation (and subsequently, the fear of being exploited) out of the picture, agents move towards mutual cooperation. 
Figure~\ref{fig:rl_imaginative_learning} shows the idea behind $SQLoss$. 

\subsubsection{$SQLoss$: Formulation}
We describe below the formulation of SQLoss with respect to agent 1. The formulation for agent 2 is identical to that of agent 1.
Let $\uptau_a = (s_{0}, u_{0}^{1}, u_{0}^{2}, r_{0}^{1}, \cdots s_{T}, u_{T}^{1}, u_{T}^{2}, r_{T}^{1})$ denote the collection of an agent's experiences after $T$ time steps.
Let $R_{t}^{1} (\uptau_1)$ denote the discounted future return for agent $1$ starting at $s_t$ in actual game-play.
Let $\hat \uptau_{1}$ denote denote the collection of an agent's \textbf{imagined} experiences. 
For a state $s_{t}$ ($t \in [0, T)$), an agent imagines an episode by starting at $s_{t}$ and repeating $u_{t-1}^{1}, u_{t-1}^{2}$ for $\kappa_{t}$ steps.
This is equivalent to imagining a $\kappa_{t}$ step repetition of already played actions. 
We sample $\kappa_{t}$ from a Discrete Uniform distribution $\mathbb{U} \{1,z\}$ where $z$ is a hyper-parameter $\geq 1$.
To simplify notation, let $\phi_t(s_t, \kappa_{t})$ denote the ordered set of state, actions, and rewards starting at time $t$ and repeated $\kappa_{t}$ times for imagined game-play.
Let $\hat R_{t}^{1} (\hat \uptau_1)$ denote the discounted future return starting at $s_t$ in imagined status-quo game-play.
% \vspace{-8pt}
{
% \setlength{\belowdisplayskip}{0pt} \setlength{\belowdisplayshortskip}{0pt}
% \setlength{\abovedisplayskip}{0pt} \setlength{\abovedisplayshortskip}{0pt}
\begin{multline}%
    \tiny
    \phi_t(s_t,\kappa_{t}) = \big[ (s_{t}, u_{t-1}^{1}, u_{t-1}^{2}, r_{t-1}^{1})_0, \cdots, \\
    (s_{t}, u_{t-1}^{1}, u_{t-1}^{2}, r_{t-1}^{1})_{\kappa_{t}-1} \big]
    % \label{eq:tau_hat_phi}
\end{multline}
% \vspace{-8pt}
\begin{multline}
    \tiny
    \hat \uptau_{1} = \big( \phi_t(s_t,\kappa_{t}), (s_{t+1}, u_{t+1}^{1}, u_{t+1}^{2}, r_{t+1}^{1})_{\kappa_{t} + 1}, \cdots, \\
    (s_{T}, u_{T}^{1}, u_{T}^{2}, r_{T}^{1})_{T+\kappa_{t}-t} \big)
    % \label{eq:tau_hat}
\end{multline}%

}


% \vspace{-8pt}
{
% \setlength{\belowdisplayskip}{0pt} \setlength{\belowdisplayshortskip}{0pt}
% \setlength{\abovedisplayskip}{0pt} \setlength{\abovedisplayshortskip}{0pt}
\begin{equation}
    \small
    \begin{split}
        R_{t}^{1} (\uptau_1) & = \sum_{l=t}^{T} \gamma^{l-t} r_{l}^{1} \\
        \hat R_{t}^{1} (\hat \uptau_1) & = \Big( \frac{1 - \gamma^{\kappa}}{1 - \gamma} \Big) r_{t-1}^{1} + \gamma^{\kappa} R_{t}^{1} (\uptau_1) \\
        & = \Big( \frac{1 - \gamma^{\kappa}}{1 - \gamma} \Big) r_{t-1}^{1} + \gamma^{\kappa} \sum_{l=t}^{T} \gamma^{l-t} r_{l}^{1}
    \end{split}
\end{equation}
}

$V_{\theta^{1},\theta^{2}}^{1}$ and $\hat V_{\theta^{1},\theta^{2}}^{1}$ are approximated by $\E [R_{0}^{1} (\uptau_1)]$ and $\E[\hat R_{0}^{1} (\hat \uptau_1)]$ respectively. 
These $V$ values are the expected rewards conditioned on both agents' policies ($\pi^{1}$, $\pi^{2}$). 
For agent 1, the regular gradients and the Status-Quo gradients,
$\nabla_{\theta^{1}} \E [R_{0}^{1}(\uptau_1)]$ and $\nabla_{\theta^{1}} \E [\hat R_{0}^{1}(\hat \uptau_1)]$, can be derived from the policy gradient formulation as:
\begin{equation}
    % \tiny
    \begin{split}
        \nabla_{\theta^{1}} \E [R_{0}^{1}(\uptau_1)] = \E & [R_{0}^{1}(\uptau_1)\nabla_{\theta^{1}} log\pi^{1}(\uptau_1)] \\
%
        = \E {\Big[} & \sum_{t=0}^{T} \nabla_{\theta^{1}} log\pi^{1} (u_{t}^{1}|s_{t}) \cdot \sum_{l=t}^{T} \gamma^{l} r_{l}^{1} {\Big]} \\
%
        = \E {\Big[} & \sum_{t=0}^{T} \nabla_{\theta^{1}} log\pi^{1} (u_{t}^{1}|s_{t}) \gamma^{t} \big( R_{t}^{1}(\uptau_1) - b(s_{t}) \big) \Big] \end{split}
\end{equation}%
\begin{equation}%
    % \tiny
    \begin{split}%
        \nabla_{\theta^{1}} \E [\hat R_{0}^{1}(\hat \uptau_1)] & = \E~[\hat R_{0}^{1}(\hat \uptau_1)\nabla_{\theta^{1}} log\pi^{1}(\hat \uptau_1)] \\
% \cdot
        = \E {\Bigg[} \sum_{t=0}^{T} & \nabla_{\theta^{1}} log\pi^{1} (u_{t-1}^{1}|s_{t}) \times \\
        & ~~~~~~~~~~~~~~~~~~~~~\Bigg( \sum_{l=t}^{t+\kappa} \gamma^{l} r_{t-1}^{1} + \sum_{l=t}^{T} \gamma^{l+\kappa} r_{l}^{1} \Bigg) \Bigg] \\
%
        = \E {\Bigg[} \sum_{t=0}^{T} & \nabla_{\theta^{1}} log\pi^{1} (u_{t-1}^{1}|s_{t}) \times \\
        & ~~~~~~~~~\Bigg( \Big( \frac{1 - \gamma^{\kappa}}{1 - \gamma} \Big) \gamma^{t} r_{t-1}^{1} + \gamma^{\kappa} \sum_{l=t}^{T} \gamma^{l} r_{l}^{1} \Bigg) \Bigg] \\
%
        = \E {\Big[} \sum_{t=0}^{T} & \nabla_{\theta^{1}} log\pi^{1} (u_{t-1}^{1}|s_{t}) \gamma^{t} \big( \hat R_{t}^{1}(\hat \uptau_1) - b(s_{t}) \big) \Big]
    \end{split}
    \label{eq:gradient_equation}
\end{equation}
    


where $b(s_{t})$ is a baseline for variance reduction.

Then the update rule $f_{sql,pg}$ for the policy gradient-based Status-Quo Learner (SQL-PG) is,
% \vspace{-4pt}
\begin{equation}
    \small
    f_{sql,pg}^{1} = \big( \alpha \cdot \nabla_{\theta^{1}} \E [R_{0}^{1}(\uptau_1)] + \beta \cdot \nabla_{\theta^{1}} \E [\hat R_{0}^{1}(\uptau_1)] \big) \cdot \delta
\end{equation}
% \vspace{-2pt}
where $\alpha$ and $\beta$ denote the loss scaling factor for the reinforce and the imaginative game-play, respectively.


\subsection{\ipdistill: Moving Beyond Iterated Matrix Games}
\label{sec:GameDistill}
In the previous sections, we have focused on evolving cooperative behavior in the iterated matrix game formulation of sequential social dilemmas. 
In the iterated matrix game formulation, an agent is only allowed to either cooperate or defect in each iteration.
However, in a social dilemma game with visual observations, it is not clear what set of low-level actions constitute cooperative or selfish behavior. 
Therefore, to work on social dilemmas with visual observations, we propose \ipdistill, an approach that automatically learns a cooperation and a defection policy by analyzing the behavior of randomly initialized agents.  
\ipdistill learns these policies in the form of cooperation and defection oracles. 
Given a state, the cooperation oracle suggests an action that represents cooperative behavior. 
Similarly, the defection oracle suggests an action that represents selfish behavior (Figure~\ref{fig:oracle_predictions} (Appendix~\ref{appendix:oracle:illustration})). 
When RL agents play the social dilemma game, each agent independently runs \ipdistill before playing the game. 
Once both agents have run \ipdistill, they consult either of the two extracted oracles in every step of the game. 
Therefore, in each step, an agent either takes the action recommended by the cooperation oracle or the action recommended by the defection oracle.
In this way, we reduce the visual input game to an iterated matrix game and subsequently apply $SQLoss$ to evolve cooperative behavior. 
\ipdistill (see Figure~\ref{fig:high_level_approach}) works as follows. 
\begin{enumerate}
    \item 
    We initialize RL agents with random weights and play them against each other in the game. 
    In these random game-play episodes, whenever an agent receives a reward, we store the sequence of the last three states up to the current state. 
    \item
    This collection of state sequences is used to train the \ipdistill network. 
    The \ipdistill network takes as input a sequence of states and predicts the rewards of both agents as well as environment parameters that depend on the game. 
    For instance, in the Coin Game, the \ipdistill network predicts the rewards of both agents and the color of the picked coin.
    \item 
    Training the \ipdistill network leads to the emergence of feature embeddings for the various state sequences. Subsequently, clustering these embeddings using Agglomerative Clustering (with number of clusters=2) leads to the development of cooperative and defection clusters. One of the learned clusters contains state sequences that represent cooperative behavior, and the other cluster contains state sequences that represent defection.
    For instance, in the Coin Game, a point in the cooperation cluster contains a sequence of states where an agent picks a coin of its color. 
    \item
    To train the cooperation and defection oracle networks, we use the collection of state sequences in each cluster. 
    For each sequence of states in a cluster, we train the oracle network to predict the next action, given the current state. 
    For instance, Figure~\ref{fig:oracle_predictions} (Appendix~\ref{appendix:oracle:illustration})shows the cooperation and defection oracles extracted by the Red agent using \ipdistill in the Coin Game.
     
\end{enumerate}

Section~\ref{sec:experimental-setup:gamedistill} describes the architectural choices of each component of \ipdistill. 
 
\begin{comment}
For any game, the idea is summarized as follows:
\begin{enumerate}
    \item \textbf{N complex actions -> M complex skills:} Learning decoupled skills has multiple benefits as they can be easily transferred to other agents, or new skills can be learned, or skills can be updated.  This also decouples the environment-specific information from the skills of the agents.
    \item \textbf{Action Prediction Network:} Once the skills are identified, this module converts the meta-learning (in the form of skill) to environment-specific actions/interactions. This allows the agents to behave a certain way in the environment given a skill.
    \item \textbf{Skill selection policy:} Given agents can interact with the environment given a skill/policy, now the task boils down to selecting a skill at a given state that maximizes the overall reward of the agents.
\end{enumerate}
\end{comment}


\begin{comment}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{images/meta_policy.png}
    \caption{Reduction of a game to an IPD formulation. We summarize complex skills using oracles and the agent has to learn a meta-policy to switch between skills. \todopb{Make a formal version of this reduction}}
    \label{fig:meta_policy}
\end{figure}

\end{comment}



==> Multi-Agent ICLR -- arxiv - updated/checklist.tex <==
\section{Reproducibility Checklist}
We follow the reproducibility checklist from \href{https://www.cs.mcgill.ca/~jpineau/ReproducibilityChecklist.pdf~}~\cite{reproducibility_checklist} and include further details here. For all the models and algorithms we have included details that we think would be useful for reproducing the results of this work.
\begin{itemize}
\item For all \textbf{models} and \textbf{algorithms} presented, check if you include:
\begin{enumerate}
    \item \textit{A clear description of the mathematical setting, algorithm, and/or model}: \textbf{Yes}. The algorithm is described in detail in Section~\ref{sec:approach}, with all the loss functions used for training being clearly defined. The details of the architecture, hyperparameters used and other algorithm details are given in Section~\ref{sec:experimental_setup}. Environment details are explained in the sections that they are introduced in.
    \item \textit{An analysis of the complexity (time, space, sample size) of any algorithm}: \textbf{No}. We do not include a formal complexity analysis of our algorithm. However, we do highlight the additional computational steps (in terms of losses and parameter updates) in Section~\ref{sec:approach} over standard multi-agent independently learning RL algorithms that would be needed in our approach.
    \item \textit{A link to a downloadable source code, with specification of all dependencies, including external libraries.}: \textbf{Yes}. We have made the source code available at \citet{github_code}.
\end{enumerate}
 
 
 
\item For any \textbf{theoretical claim}, check if you include:
\begin{enumerate}
    \item \textit{A statement of the result}: \textbf{NA}. Our paper is primarily empirical and we do not have any major theoretical claims. Hence this is Not Applicable.
    \item \textit{A clear explanation of any assumptions}: \textbf{NA}.  
    \item \textit{A complete proof of the claim}: \textbf{NA}.
\end{enumerate}
 
\item For all \textbf{figures} and \textbf{tables} that present empirical results, check if you include:
\begin{enumerate}
    \item \textit{A complete description of the data collection process, including sample size}: \textbf{NA}. We did not collect any data for our work.
    \item \textit{A link to a downloadable version of the dataset or simulation environment}: \textbf{Yes}. We have made the source code available at \citet{github_code}.
    \item \textit{An explanation of any data that were excluded, description of any pre-processing step}: \textbf{NA}. We did not perform any pre-processing step.
    \item \textit{An explanation of how samples were allocated for training / validation / testing}: \textbf{Yes}. For \ipdistill the details regarding data used for training is given in Section~\ref{sec:GameDistill}. The number of iterations used for learning (training) by $SQLearner$ is given in Figures~\ref{fig:results_IPD},~\ref{fig:results_IMP} and~\ref{fig:coingame_results}. The details of the number of runs and the batch sizes used for various experiments are given in Section~\ref{sec:experimental_setup}.
    \item \textit{The range of hyper-parameters considered, method to select the best hyper-parameter configuration, and specification of all hyper-parameters used to generate results}: \textbf{Yes}. We did not do any hyperparameter tuning as part of this work. All the hyperparameters that we used are specified in Section~\ref{sec:experimental_setup}.
    \item \textit{The exact number of evaluation runs}: \textbf{Yes}. For all our environments, we repeat the experiment $20$ times. For evaluation of performance, we use an average of $200$ Monte Carlo estimates. We state this in Section~\ref{sec:experimental_setup}. We do not fix any seeds. The details of the number of runs and the batch sizes used for various experiments are also given here.
    \item \textit{A description of how experiments were run}: \textbf{Yes}. The README with instructions on how to run the experiments along with the source code is provided at~\citet{github_code}.
    \item \textit{A clear definition of the specific measure or statistics used to report results}: \textbf{Yes}. We plot the mean and the one standard deviation region over the mean for all our numerical experiments. This is stated in Section~\ref{sec:experimental_setup}.
    \item \textit{Clearly defined error bars}: \textbf{Yes}. We plot the mean and the one standard deviation region over the mean for all our numerical experiments. This is stated in Section~\ref{sec:experimental_setup}.
    \item \textit{A description of results with central tendency (e.g. mean) \& variation (e.g. stddev)}: \textbf{Yes}. We plot the mean and the one standard deviation region over the mean for all our numerical experiments. This is stated in Section~\ref{sec:experimental_setup}.
    \item \textit{A description of the computing infrastructure used}: \textbf{Yes}. We have provided this detail in the Supplementary material in Section~\ref{sec:sup_arch}.
\end{enumerate}
\end{itemize}

==> Multi-Agent ICLR -- arxiv - updated/conclusion.tex <==
\section{Conclusion}
We have described a status-quo loss ($SQLoss$) that encourages an agent to imagine the consequences of sticking to the status-quo.
We demonstrated how agents trained with $SQLoss$ evolve cooperative behavior in several social dilemmas without sharing rewards, gradients, or using a communication channel. 
To work with visual input games, we proposed $GameDistill$, an approach that automatically extracts a cooperative and a selfish policy from a social dilemma game.
We combined $GameDistill$ and $SQLoss$ to demonstrate how agents evolve desirable cooperative behavior in a social dilemma game with visual observations.
\label{sec:conclusion}



==> Multi-Agent ICLR -- arxiv - updated/experimental_setup.tex <==
\section{Experimental Setup}
\label{sec:experimental_setup}

\begin{table*}
    \centering
    \small
    \begin{subtable}[t]{0.3\linewidth}
        \centering
        \renewcommand{\arraystretch}{1.2}
        \begin{tabular}{c|c|c}
             & $C$ & $D$ \\ \hline
             $C$ & (-1, -1) & (-3, 0) \\ \hline
             $D$ & (0, -3) & (-2, -2) \\ \hline
        \end{tabular}
        \caption{Prisoners' Dilemma (PD)}
        \label{tab:payoff_matrix_ipd}
    \end{subtable}%
    \begin{subtable}[t]{0.3\linewidth}
        \centering
        \renewcommand{\arraystretch}{1.2}
        \begin{tabular}{c|c|c}
             & $H$ & $T$ \\ \hline
             $H$ & (+1, -1) & (-1, +1) \\ \hline
             $T$ & (-1, +1) & (+1, -1) \\ \hline
        \end{tabular}
        \caption{Matching Pennies (MP)}
        \label{tab:payoff_matrix_imp}
    \end{subtable}%
    \begin{subtable}[t]{0.3\linewidth}
        \centering
        \renewcommand{\arraystretch}{1.2}
        \begin{tabular}{c|c|c}
             & $C$ & $D$ \\ \hline
             $C$ & (0, 0) & (-4, -1) \\ \hline
            %  $C$ & (4, 4) & (0, 3) \\ \hline
             $D$ & (-1, -4) & (-3, -3) \\ \hline
            %  $D$ & (3, 0) & (1, 1) \\ \hline
        \end{tabular}
        \caption{Stag Hunt (SH)}
        \label{tab:payoff_matrix_sh}
    \end{subtable}%
    
    \caption{\label{tab:payoff_matrix}%
    Payoff matrices for the different games used in our experiments. 
    $(X,Y)$ in a cell represents a reward of $X$ to the row and $Y$ to the column player. 
    $C$, $D$, $H$, and $T$ denote the actions for the row and column players.
    In the iterated versions of these games, agents play against each other over several iterations. 
    In each iteration, an agent takes an action and receives a reward based on the actions of both agents. 
    Each matrix represents a different kind of social dilemma.
    }
\end{table*}

In order to compare our results to previous work~\cite{foerster2018learning}, we use the Normalized Discounted Reward ($NDR = (1-\gamma) \sum_{t=0}^{T} \gamma^{t} r_{t}$). 
A higher NDR implies that an agent obtains a higher reward in the environment. 
We compare our approach (Status-Quo Aware Learner: $SQLearner$) to Learning with Opponent-Learning Awareness (Lola-PG)~\cite{foerster2018learning} and the Selfish Learner (SL, Section~\ref{sec:approach:selfish-learner}).
For all experiments, we perform $20$ runs and report average $NDR$, along with variance across runs.
The bold line in all the figures is the mean, and the shaded region is the one standard deviation region over the mean. 
All of our code is available at~\citet{github_code}.

\subsection{Social Dilemma Games}
For our experiments with social dilemma matrix games, we use the (Iterated Prisoners Dilemma (IPD)~\cite{luce1989games}, Iterated Matching Pennies (IMP)~\cite{lee1967application}, and the Iterated Stag Hunt (ISH)~\cite{foerster2018learning}). 
Table~\ref{tab:payoff_matrix} shows the payoff matrix for a single iteration of each game. 
In iterated matrix games, at each iteration, agents take an action according to a policy and receive the rewards in Table~\ref{tab:payoff_matrix}.
To simulate an infinitely iterated game, we let agents play 200 iterations of the game against each other, and do not provide an agent with any information about the number of remaining iterations~\cite{foerster2018learning}. 
In an iteration, the state for an agent is the actions played by both agents in the previous iteration. 
Each matrix game in Table~\ref{tab:payoff_matrix} represents a different dilemma. 

In the Prisoner's Dilemma, the rational policy for each agent is to defect, regardless of the policy of the other agent.  
However, when each agent plays rationally, each is worse off. 
In Matching Pennies, if an agent plays predictably, it is prone to exploitation by the other agent.
Therefore, the optimal policy is to randomize between $H$ and $T$, obtaining an average NDR of $0$.
The Stag Hunt game represents a coordination dilemma. 
In the game, given that the other agent will cooperate, an agent's optimal action is to cooperate as well. 
However, at each step, each agent has an attractive alternative, that of defecting and obtaining a guaranteed reward of $3$. 
Therefore, the promise of a safer alternative and the fear that the other agent might select the safer choice could drive an agent to also select the safer alternative, thereby sacrificing the higher reward of mutual cooperation. 

For our experiments on a social dilemma with visual observations, we use the Coin Game (Figure~\ref{fig:coin_game}) \cite{foerster2018learning}.
The rational policy for an agent is to defect and try to pick all coins, regardless of the policy of the other agent.
However, when both agents defect, both are worse off. 

\subsection{SQLoss}
For our experiments with the Selfish and Status-Quo Aware Learner ($SQLearner$), we use policy gradient-based learning where we train an agent with the Actor-Critic method~\cite{sutton2011reinforcement}. 
Each agent is parameterized with a policy actor and critic for variance reduction in policy updates. 
During training, we use gradient descent with step size, $\delta = 0.005$ for the actor and $\delta = 1$ for the critic. 
We use a batch size of $4000$ for Lola-PG~\cite{foerster2018learning} and 200 for $SQLearner$ for roll-outs. 
We use an episode length of 200 for all iterated matrix games. 
We use a discount rate ($\gamma$) of $0.96$ for the Iterated Prisoners' Dilemma, Iterated Stag Hunt, and Coin Game. 
For the Iterated Matching Pennies, we use $\gamma = 0.9$.
The high value of $\gamma$ allows for long time horizons, thereby incentivizing long-term reward. 
Each agent randomly samples $\kappa$ from $\mathbb{U} \in (1, z)$ ($z=10$, discussed in Appendix~\ref{appendix:effect-z-convergence}) at each step.



\subsection{GameDistill}
\label{sec:experimental-setup:gamedistill}

\ipdistill consists of two components.
First, the state sequence encoder (Step 2, Section~\ref{sec:GameDistill}) that takes as input a sequence of states and outputs a feature representation. 
We encode each state in the sequence using a series of standard Convolution layers with kernel-size 3. 
We then use a fully-connected layer with 100 neurons that outputs a dense representation of the sequence of states.
The color of picked coin, agent reward, and opponent reward branches consist of a series of dense layers with linear activation.
We use linear activation so that we can cluster the feature vectors (embeddings) using a linear clustering algorithm, such as Agglomerative Clustering. 
We obtain similar results when we use the K-means clustering algorithm. 
We use the \textit{Binary-Cross-Entropy (BCE)} loss for classification and the \textit{mean-squared error (MSE)} loss for regression. 
We use the \textit{Adam}~\cite{kingma2014adam} optimizer (learning rate $0.003$).

Second, the oracle network (Step 4, Section~\ref{sec:GameDistill}), that predicts an action for an input state. 
We encode the input state using $2$ convolution layers with kernel-size $3$ and \textit{relu} activation. 
To predict the action, we use $3$ fully-connected layers with \textit{relu} activation and the BCE loss.
We use \textit{L2} regularization, and \textit{Gradient Descent} with the \textit{Adam} optimizer (learning rate $0.001$).



==> Multi-Agent ICLR -- arxiv - updated/introduction.tex <==
\section{Introduction}
\label{sec:introduction}


\begin{comment}
\begin{figure}[ht]
    \includegraphics[width=\linewidth]{images/overall_idea.png}
    \caption{A schematic diagram of the proposed idea}
    \label{fig:overall_idea}
\end{figure}
\end{comment}
% In intertemporal social dilemmas, there is a tradeoff between short-term individual incentives and long-term collective interest. Humans face such dilemmas when contributing to a collective food storage during the summer in preparation for a harsh winter, organizing annual maintenance of irrigation systems, or sustainably sharing a local fishery. Classical models of human behavior based on rational choice theory predict that cooperation in these situations is impossible [1, 2]. This poses a puzzle since humans evidently do find ways to cooperate in many everyday intertemporal social dilemmas, as documented by decades of fieldwork [3, 4] and laboratory experiments [5, 6]. Providing an empirically grounded explanation of how individual behavior gives rise to societal cooperation is seen as a core goal in several subfields of the social sciences and evolutionary biology [7, 8, 9].[10, 11] proposed influential models based on behavioral game theory. However, these models have limited applicability since they only generate predictions when the problem can be cast as a matrix game (see e.g. [12, 13]). Here we consider a more realistic video-game setting, like those introduced in the behavioral research of [14, 15, 16]. In this environment, agents do not simply choose to cooperate or defect like they do in matrix games. Rather they must learn policies to implement their strategic decisions, and must do so while coping with the non-stationarity arising from other agents learning simultaneously. Several papers used multi-agent reinforcement learning [17, 18, 19] and planning [20, 21, 22, 23] to generate cooperation in this setting. However, this approach has not yet demonstrated robust cooperation in games with more than two players, which is often observed in human behavioral experiments. Moreover naïvely optimizing group reward is also ineffective, due to the lazy agent problem [24].
%It is difficult for both natural and artificial agents to find cooperative solutions to intertemporal social dilemmas for the following reasons:
%1. Collective action – individuals must learn and coordinate policies at a group level to avoid falling into socially deficient equilibria.
%2. Temporal credit assignment – rational defection in the short-term must become associated with long-term negative consequences.
%Many different research traditions, including economics, evolutionary biology, sociology, psychology, and political philosophy have all converged on the idea that fairness norms are involved in resolving social dilemmas [25, 26, 27, 28, 29, 30, 31]. In one well-known model, agents are assumed to have inequity-averse preferences [10]. They balance their selfish desire for individual rewards against a need to keep deviations between their own rewards and the rewards of others as small as possible. Inequity-averse individuals are able to solve social dilemmas by resisting the temptation to pull ahead of others or—if punishment is possible—by punishing and discouraging free-riding. The inequityaversion model has been successfully applied to explain human behavior in a variety of laboratory economic games, such as the ultimatum game, the dictator game, the gift exchange game, market games, the trust game and public goods

%Google paper
% Social dilemmas expose tensions between collective and individual rationality [1]. Cooperation makes possible better outcomes for all than any could obtain on their own. However, the lure of free riding and other such parasitic strategies implies a tragedy of the commons that thrickens the stability of any cooperative venture [2]. 
%The theory of repicked general-sum matrix games provides a framework for understanding social dilemmas. Fig. 1 shows payoff matrices for three canonical examples: Prisoner's Dilemma, Chicken, and Stag Hunt. The two actions are interpreted as cooperate and defect respectively. The four possible outcomes of each stage game are R (reward of mutual cooperation), P (punishment arising from mutual defection), S (sucker outcome obtained by the player who cooperates with a defecting partner), and T (temptation outcome achieved by defecting against a cooperator).
%A matrix game is a social dilemma when its four payoffs satisfy the following social dilemma inequalities (this formulation from [3]):
%1. R > P Mutual cooperation is preferred to mutual defection. (1)
%2. R > S Mutual cooperation is preferred to being exploited by a defector. (2)
%3. 2R > T +S This ensures that mutual cooperation is preferred to an equal probability of unilateral cooperation and defection. (3)
%4. either greed: T > R Exploiting a cooperator is preferred over mutual cooperation or fear: P > S Mutual defection is preferred over being exploited. (4)
%Matrix Game Social Dilemmas (MGSD) have been fruitfully employed as models for a wide variety of phenomena in theoretical social science and biology.



Consider a sequential social dilemma, where individually rational behavior leads to outcomes that are sub-optimal for each individual in the group. \cite{Hardin1968,ostrom:1990,Ostrom278,Dietz1907}. 
Current state-of-the-art Multi-Agent Deep Reinforcement Learning (MARL) methods that train agents independently can lead to agents that fail to cooperate reliably, even in simple social dilemma settings. 
This failure to cooperate results in sub-optimal individual and group outcomes (\citet{foerster2018learning, Peysakhovich1707.01068}, Section~\ref{sec:approach:selfish-learner}). 

To illustrate why it is challenging to evolve cooperation in such dilemmas, we consider the Coin Game (\cite{foerster2018learning}, Figure~\ref{fig:coin_game}). 
Each agent can play either selfishly (pick all coins) or cooperatively (pick only coins of its color). 
Regardless of the behavior of the other agent, the individually rational choice for an agent is to play selfishly, either to minimize losses (avoid being exploited) or to maximize gains (exploit the other agent).  
However, when both agents behave rationally, they try to pick all coins and achieve an average long term reward of $-0.5$. 
In contrast, if both play cooperatively, then the average long term reward for each agent is $0.5$.
Therefore, when agents cooperate, they are both better off. 
Training Deep RL agents independently in the Coin Game using state-of-the-art methods leads to mutually harmful selfish behavior (Section~\ref{sec:approach:selfish-learner}).  


In this paper, we present a novel MARL algorithm that allows independently learning Deep RL agents to converge to \textbf{individually and socially desirable cooperative behavior} in such social dilemma situations. 
Our key contributions can be summarised as:
\begin{enumerate}
    \item We introduce a \textbf{Status-Quo} loss ($SQLoss$, Section~\ref{sec:approach:SQLoss}) and an associated policy gradient-based algorithm to evolve optimal behavior for agents that can act in either a cooperative or a selfish manner, by choosing between a cooperative and a selfish policy. 
     We empirically demonstrate that agents trained with the $SQLoss$ evolve optimal behavior in several social dilemma iterated matrix games (Section \ref{sec:results}).
    \item We propose \ipdistill (Section~\ref{sec:GameDistill}), an algorithm that reduces a social dilemma game with visual observations to an iterated matrix game by extracting policies that implement cooperative and selfish behavior.  
    We empirically demonstrate that \ipdistill extracts cooperative and selfish policies for the Coin Game (Section~\ref{sec:results:visual-input-gamedistll-and-sqloss}). 
    \item We demonstrate that when agents run \ipdistill followed by MARL game-play using $SQLoss$, they converge to individually as well as socially desirable cooperative behavior in a social dilemma game with visual observations (Section~\ref{sec:results:visual-input-gamedistll-and-sqloss}).
\end{enumerate}

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{images/coin_game_dynamics.pdf}
    \caption{
    Two agents (Red and Blue) playing the Coin Game. 
    The agents, along with a Blue or Red coin, appear at random positions in a 3x3 grid. 
    An agent observes the complete 3x3 grid as input and can move either left, right, up, or down.
    When an agent moves into a cell with a coin, it picks the coin, and a new instance of the game begins.
    If the Red agent picks the Red coin, it gets a reward of $+1$ and the Blue agent gets no reward.
    If the Red agent picks the Blue coin, it gets a reward of $+1$, and the Blue agent gets a reward of $-2$.
    The blue agent's reward structure is symmetric to that of the red agent.
    }
    \label{fig:coin_game}
\end{figure}

The problem of how independently learning agents evolve cooperative behavior in social dilemmas has been studied by researchers through human studies and simulation models~\cite{Fudenberg, Edward:1984, Fudenberg:1984, Kamada:2010, Abreu:1990}. 
A large body of work has looked at the mechanism of evolution of cooperation through reciprocal behaviour and indirect reciprocity~\cite{reciprocal1971,reciprocal1984,reciprocal1992,reciprocal1993,in_reciprocal1998}, through variants of reinforcement using aspiration~\cite{reinforce_variant}, attitude~\cite{NonRL_attitude} or multi-agent reinforcement learning~\cite{Sandholm1996MultiagentRL,Wunder:2010}, and under specific conditions~\cite{R_plus_S_g_2P} using different learning rates \cite{deCote:2006} similar to WoLF~\cite{WOLF2002} as well as using embedded emotion~\cite{Emotional_Multiagent}, social networks~\cite{Ohtsuki2006,Santos:2006}.

However, these approaches do not directly apply to Deep RL agents~\cite{Leibo:2017}.
Recent work in this direction~\cite{kleiman2016coordinate,Julien:2017,consequentialist18} focuses on letting agents learn strategies in multi-agent settings through interactions with other agents.  
\citet{Leibo:2017} define the problem of social dilemmas in the Deep RL framework and analyze the outcomes of a fruit-gathering game~\cite{Julien:2017}.
They vary the abundance of resources and the cost of conflict in the fruit environment to generate degrees of cooperation between agents. 
\citet{Hughes:2018} define an intrinsic reward (inequality aversion) that attempts to reduce the difference in obtained rewards between agents. 
The agents are designed to have an aversion to both advantageous (guilt) and disadvantageous (unfairness) reward allocation. 
This handcrafting of loss with mutual fairness evolves cooperation, but it leaves the agent vulnerable to exploitation.
LOLA~\cite{foerster2018learning} uses opponent awareness to achieve high levels of cooperation in the Coin Game and the Iterated Prisoner's Dilemma game.
However, the LOLA agent assumes access to the other agent's policy parameters and gradients. 
This level of access is analogous to getting complete access to the other agent's private information and therefore devising a strategy with full knowledge of how they are going to play. 
\citet{Wang:2019} propose an evolutionary Deep RL setup to evolve cooperation. 
They define an intrinsic reward that is based on features generated from the agent's past and future rewards, and this reward is shared with other agents. They use evolution to maximize the sum of rewards among the agents and thus evolve cooperative behavior. 
However, sharing rewards in this indirect way enforces cooperation rather than evolving it through independently learning agents. 


In contrast, we introduce a Status-Quo ($SQLoss$) that evolves cooperation between agents without sharing rewards, gradients, or using a communication channel. 
The $SQLoss$ encourages an agent to imagine the consequences of sticking to the status-quo.
This imagined stickiness ensures that an agent gets a better estimate of a cooperative or selfish policy.
Without $SQLoss$, agents repeatedly switch policies (from cooperative to selfish), obtain short-term rewards (through exploitation), and, therefore incorrectly learn that a selfish strategy gives higher rewards in the long-term.  
\todopb{Figure~??? shows how $SQLoss$ compares to existing approaches to evolve cooperative behavior in multi-agent reinforcement learning games.} 

To work with social dilemma games that have visual observations, we introduce \ipdistill.
\ipdistill uses self-supervision and clustering to automatically extract a cooperative and a selfish policy from a social dilemma game.
The input to \ipdistill is a collection of state sequences derived from game-play between two randomly initialized agents. 
Each state sequence represents a collection of states and actions (of both agents), leading up to a reward in the environment.  
\ipdistill uses this collection of state sequences to learn two oracles.
One oracle represents a cooperative policy, and the other oracle represents a selfish policy.
Given a state, an oracle returns an action according to the specific policy.  
It is important to note that each agent independently runs \ipdistill to extract oracles. 
(For instance, Figure~\ref{fig:oracle_predictions} (Appendix~\ref{appendix:oracle:illustration}) illustrates the cooperation and defection oracles extracted by the Red agent using \ipdistill in the Coin Game.)
Figure~\ref{fig:high_level_approach} shows the high-level architecture of our approach.

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{images/high_level_approach_new_horizontal.pdf}
    \caption{
    High-level architecture of our approach.
    Each agent runs \ipdistill by performing $(1), (2), (3)$ individually before playing the social dilemma game. This creates two oracles per agent.
    During game-play$(4)$, each agent (enhanced with $SQLoss$) takes either the action suggested by the cooperation oracle or the action suggested by the defection oracle. 
    }
    \label{fig:high_level_approach}
\end{figure*}

\begin{enumerate}
    \item For a social dilemma game with visual observations, each RL agent runs \ipdistill to learn oracles that implement cooperative and selfish behavior. 
    \item We train agents (with $SQLoss$) to play the game such that at any step, an agent can either take the action suggested by the cooperation oracle or the selfish oracle. 
\end{enumerate}

We empirically demonstrate in Section~\ref{sec:results} that our approach evolves cooperative behavior between independently trained agents. 




\begin{comment}
This result is particularly interesting because behavioral economists~\cite{samuelson1988status, kahneman1991anomalies, kahneman2011thinking, thaler2009nudge} have studied the effect of the Status-Quo bias in decision making in humans. 
Our work shows that it is possible that the Status-Quo bias helps to evolve cooperative behavior in human groups.

They start with two policies, cooperation (denoted by $\pi_C$) and defection (denoted by $\pi_D$). 
They use these policies to generate intermediate policies with varying degrees of Cooperation and Defection. 
During game-play, each agent predicts the degree of cooperation of its opponent and chooses a policy of the same degree of cooperation. 
We propose an IPD-Distilling architecture (\ipdistill) to transform a multi-agent game to its IPD formulation.
\ipdistill uses self-supervision and clustering to learn cooperation and defection policies automatically.
We use \ipdistill to transform a game to an IPD, followed by $SQLoss$ enhanced agents to evolve cooperative behavior for RL agents in the Coin game \cite{foerster2018learning}. 
We show that RL agents trained using our approach achieve higher levels of cooperation and average reward than those trained with existing approaches (Section~\ref{sec:results}).
%Figure~\ref{fig:high_level_approach} shows a high-level description of our approach. 

\end{comment}



\begin{comment}

In \cite{consequentialist18}, \citeauthor{consequentialist18} takes the direction of having predefined policies of cooperation($\pi_C$) and defection ($\pi_D$) and have built in a handcrafted mechanism of playing multiple rollouts of actions $CC$ and $CD$ to figure out the payoffs for these strategies. Subsequently, they use a rule based mechanism to choose between cooperation($\pi_C$) and defec`                                                                                                                                                                                                                                                                                                                                 tion ($\pi_D$) policies. Their idea of having existing policies of ($\pi_C$) and ($\pi_D$) is similar to our idea of learning skills of cooperation or defection. However, we try to discover these policies using a self-supervised clustering method while playing the game in a random manner (i.e. random action policy). 
\end{comment}



==> Multi-Agent ICLR -- arxiv - updated/related_work.tex <==
\section{Related Work}
\label{sec:related_work}
Social dilemma problems brings out the conflict between an individual and the society and
Prisoner's dilemma \cite{Rapoport1974} has been used to highlight this core conflict. In-spite of several examples of cooperation in nature at various scales, from microscopic \cite{Szathmary1995}, to species level \cite{Heinsohn1995ComplexCS} including humans\cite{kleiman2016coordinate}, still greedy behavior leads to tragedy of the commons \cite{psychology_social_dilemmas}

There has been a large body of work which had looked at the mechanism of emergence of cooperation through reciprocal behaviour and indirect reciprocity \cite{reciprocal1971},\cite{reciprocal1984},\cite{reciprocal1992},\cite{reciprocal1993},\cite{in_reciprocal1998}, though variants of reinforcement using aspiration \cite{reinforce_variant}, attitude\cite{NonRL_attitude} or using multi-agent reinforcement learning \cite{Sandholm1996MultiagentRL,Wunder:2010}, under specific conditions \cite{R_plus_S_g_2P}, using different learning rates \cite{deCote:2006} similar to WoLF \cite{WOLF2002} as well as using embedded emotion \cite{Emotional_Multiagent}.

But with the advent of deep reinforcement learning~\cite{Mnih:2013,Mnih:2015}, recent work on social dilemma problem have taken a rather hands off approach with the idea of letting agents figure out strategies, all by themselves. In the paper~\cite{Leibo:2017} the authors have setup the problem of social dilemma in deep reinforcement learning framework and have analyzed the outcome of the 2d Fruit gathering game as general sum matrix games, where by varying the abundance of resources and cost of conflict, they generate varying degrees of cooperation. In~\cite{Hughes:2018}, they define an intrinsic reward called inequality aversion which tries to reduce difference in rewards among the agents by having aversion to both advantageous(guilt) and disadvantageous(unfairness) inequity. This handcrafting of loss with mutual fairness leads to better cooperation but also makes the agent vulnerable to exploitation. The authors in~\cite{foerster2018learning} propose LOLA, where they achieve high degree of cooperation in their Coin game and Iterative Prisoner's Dilemma. They do this by having access to the opponent policy parameters and gradients. This is equivalent to getting access to opponent's brain and devising strategy with the knowledge of how they are about to play. In a more recent paper~\cite{Wang:2019}, \citeauthor{Wang:2019} proposes an evolutionary based deep reinforcement learning setup to evolve cooperation. They define an intrinsic reward which is based on a feature, generated from agent's past and expected future rewards and this feature is shared with other agents. They then use evolution to maximise the sum of rewards among the agents which leads to achieving cooperation. This is an indirect method of maximizing the sum of rewards for the society which would lead to cooperation.
Another paper \cite{Wang:2018} proposed a method, where they start with two policies, cooperation($\pi_C$) and defection ($\pi_D$). With these they generate several intermediate policies with varying degrees of ($\pi_C$) and ($\pi_D$) and then during gameplay each agent tries to predict the degree of cooperation by its opponent and chooses a matching policy of same degree of cooperation. This is an indirect way of hard coding a strategy like Tit-For-Tat because both agent try to mimic the opponent's perceived policy rather than playing to maximize their respective rewards. In contrast to these methods we try to develop cooperation using a status-quo loss, without inducing any strategy bias towards cooperation.

In \cite{consequentialist18}, \citeauthor{consequentialist18} takes the direction of having predefined policies of cooperation($\pi_C$) and defection ($\pi_D$) and have built in a handcrafted mechanism of playing multiple rollouts of actions $CC$ and $CD$ to figure out the payoffs for these strategies. Subsequently, they use a rule based mechanism to choose between cooperation($\pi_C$) and defection ($\pi_D$) policies. Their idea of having existing policies of ($\pi_C$) and ($\pi_D$) is similar to our idea of learning skills of cooperation or defection. However, we try to discover these policies using a self-supervised clustering method while playing the game in a random manner (i.e. random action policy). 

% \citet{kleiman2016coordinate} studied the emergence of cooperation and defection for humans and compare it results from agents learnt using reinforcement-learning.

==> Multi-Agent ICLR -- arxiv - updated/results.tex <==
\section{Results}
\label{sec:results}

% \label{sec:results}
% \begin{figure*}[!th]
%     \centering
%     \begin{subfigure}[t]{.5\linewidth}
%         \centering
%         \includegraphics[width=0.85\linewidth]{3d-feature-vec.png}
%         \caption{3-dimensional feature vector}
%         \label{fig:clustering_3d}
%     \end{subfigure}\hfil%
%     \begin{subfigure}[t]{.5\linewidth}
%         \centering
%         \includegraphics[width=0.85\linewidth]{images/4d-feature-vec.png}
%         \caption{4-dimensional feature vector}
%         \label{fig:clustering_4d}
%     \end{subfigure}\hfil%
%     \begin{subfigure}[t]{.5\linewidth}
%         \centering
%         \includegraphics[width=0.85\linewidth]{images/10d-feature-vec.png}
%         \caption{10-dimensional feature vector}
%         \label{fig:clustering_10d}
%     \end{subfigure}\hfil%
%     \begin{subfigure}[t]{.5\linewidth}
%         \centering
%         \includegraphics[width=0.85\linewidth]{images/100d-feature-vec.png}
%         \caption{100-dimensional feature vector}
%         \label{fig:clustering_100d}
%     \end{subfigure}%
% \caption{\label{fig:feature_vector_plots}%
% In each subfigure, Left figures represent the actual rewards obtained by both the agents (the ground-truth), while the figures on the Right represent the clusters obtained by Agglomerative Clustering (when no-of-clusters was set to 2). For feature vectors of higher dimensions (>2), we show their t-SNE~\cite{maaten2008visualizing} projections. In the figures on the left, the Legend shows the events that give $Agent_{1}$ a reward of $r_{1}$ and $Agent_{2}$ a reward of $r_{2}$ denoted in the format \textbf{$r_{1}$|$r_{2}$}. In the plots on the right, from the legend, Class $0$ and Class $1$ represent the Cooperation and Defection clusters respectively. From the figures, all the events that resulted in the opponent getting penalized belong to the same cluster, namely the Defection cluster.}
% \end{figure*}

\begin{comment}

\subsection{Learning optimal policies in Iterated Matrix Games through an $\eta$-stationary environment}



\begin{figure*}
    \centering
    \begin{subfigure}[t]{0.4\linewidth}
        \includegraphics[width=\linewidth]{images/ipd_results_sticky=5.png}
        \caption{($\eta=5$)-Stationary environment}
        \label{fig:ipd_results_sticky=5}
    \end{subfigure}\hfil%
    \begin{subfigure}[t]{0.4\linewidth}
        \includegraphics[width=\linewidth]{images/ipd_results_sticky=20.png}
        \caption{($\eta=20$)-Stationary environment}
        \label{fig:ipd_results_sticky=20}
    \end{subfigure}%
\caption{
    Instantaneous probability of cooperation for two selfish learner agents in the IPD game when the environment enforces stationarity. 
    The Green line indicates the probability of cooperation and the Blue line the probability of defection.
    When the level of stationarity enforced by the environment is high (20), even selfish learners evolve cooperation.
    }

\label{fig:ipd_results_with_sticky}%
\end{figure*}


%\begin{figure}[h]
%    \includegraphics[width=0.4\textwidth]{images/ipd_results_action_loss_at_t=1_and_t=2_sticky=10.png}
%    \caption{Instantaneous probability of cooperation for both the agents in the IPD game when the environment enforces the sticky policy with stickiness=20 and the agents are penalized only at t=2 step of the sticky game-play for action-loss.}
%    \label{fig:ipd_results_action_loss_at_t=1_and_t=2_sticky=10}
%\end{figure}
% \begin{figure}[h]
%     \includegraphics[width=0.4\textwidth]{images/ipd_results_with_futuristic_state_loss.png}
%     \caption{Average Probability of cooperation for both the agents in a traditional IPD game with the proposed imaginative-learning loss.}
%     \label{fig:ipd_results_with_futuristic_state_loss}
% \end{figure}
%\begin{figure}[h]
%    \includegraphics[width=0.4\textwidth]{images/ipd_results_with_futuristic_state_loss__variance_K=1-2.png}
%    \caption{Average Probability of cooperation for both the agents in a traditional IPD game with the proposed imaginative-learning loss with $\kappa$ varying from 1 to 2 (both inclusive).  \textcolor{green}{Green} line indicates probability of cooperation while \textcolor{blue}{Blue} line indicates probability of defection}
%    \label{fig:ipd_results_with_futuristic_state_loss__with_variance}
%\end{figure}


\paragraph{\textbf{Iterated Prisoner's Dilemma (IPD):}}
\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{images/results__IPD__nash_eq_almost.png}
    \caption{
    Average NDR values for different learners in the IPD game. 
    The reward graph for $a0$ is hidden because of overlap with the graph for $a1$. 
    $SQLearner$ agents obtain a near-optimal NDR value (-1) for this game. 
    }
    \label{fig:results_IPD}
\end{figure}


To validate our hypothesis that Selfish Learners evolve cooperative behavior in a stationary environment, we train two $SL$ agents in the IPD game using a $5$-stationary environment and a $20$-stationary environment.
Figure \ref{fig:results_IPD} shows the results.
As expected, we see that enforcing stationarity in the environment induces cooperative behavior between independently trained agents.
In the $20$-stationary environment, the probability of agents cooperating is close to 1 (agents always cooperate). 
We also observe that the probability of cooperation sharply drops every few epochs. 
We believe that these sudden drops are due to the inherent incentive to exploit the other agent. 
However, once the agents realize that mutual exploitation is harmful, they revert to cooperative behavior. 
The interval between consecutive drops in cooperation probability reduces as training proceeds.

We obtain similar results for a $10$-stationary environment; however, in this case, it took longer for the agents to converge to cooperation. 
We have omitted the figure for space considerations.
Interestingly, in the $5$-stationary environment (Figure~\ref{fig:ipd_results_sticky=5}), agents do not converge to cooperation. 
This result implies that there is a minimum environment stationarity threshold that is required for agents to overcome short-term exploitation considerations and converge to cooperation. 
For IPD, we find that this stationarity threshold is equal to ... 


%Developing motivation from the \textit{sticky policy} results, we further experiment with breaking-down stickiness to understand its impact on the learning of the agents. In a traditional IPD game, agents are penalized at each decision. However, with a sticky policy enforced in the environment, the environment ideally only requests for the action once every sticky game-play. However, penalizing only at every sticki'th step would convert it into a traditional game. We then experiment with propagating loss only at t=2 step of the sticky game-play. Fig~\ref{fig:ipd_results_action_loss_at_t=1_and_t=2_sticky=10} shows that the agents learn to cooperate with loss at just t=2 step of the sticky game-play for the action loss. Interestingly, having a mask at the action-value loss is enough to assist agents in learning to cooperate.

Figure~\ref{fig:imp_results_with_sticky} and Figure~\ref{fig:ish_results_with_sticky} in Appendix A show the probability of cooperation for $SL$ agents trained in the \textbf{IMP} and \textbf{ISH} game respectively. 
For both games, we find that agents evolve optimal policies when the environment is stationary.
\end{comment}

\subsection{Learning optimal policies in Iterated Matrix Games using SQLoss}
\label{sec:results:iterated-matrix-games:sqloss}

\paragraph{\textbf{Iterated Prisoner's Dilemma (IPD):}}
\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{images/IPD_results_corrected.png}
    \caption{\label{fig:results_IPD}%
    Average NDR values for different learners in the IPD game. 
    $SQLearner$ agents obtain a near-optimal NDR value $(-1)$ for this game. 
    In contrast to other methods, $SQLearner$ agents have close to zero variance across runs. 
    }
\end{figure}

We train different learners to play the IPD game. 
Figure~\ref{fig:results_IPD} shows the results.
For all learners, agents initially defect and move towards an NDR of $-2.0$. 
This initial bias towards defection is expected, since, for agents trained with random game-play episodes, the benefits of exploitation outweigh the costs of mutual defection.
For Selfish Learner (SL) agents, the bias intensifies, and the agents converge to mutually harmful selfish behavior (NDR=$-2.0$).  
Lola-PG agents learn to predict each other's behavior and therefore realize that defection is more likely to lead to mutual harm than selfish benefit.
They subsequently move towards cooperation, but occasionally defect (NDR=$-1.2$).
In contrast, $SQLearner$ agents quickly realize the costs of defection, indicated by the small initial dip in the NDR curves.
They subsequently move towards almost perfect cooperation, with an NDR of $-1.0$.
Finally, it is important to note that $SQLearner$ agents have close to zero variance, unlike other methods where the variance in NDR across runs is significant. 

\paragraph{\textbf{Iterated Matching Pennies (IMP):}}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/results__IMP__nash_eq_corrected.png}
    \caption{
    Average NDR values for different learners in the IMP game. 
    $SQLearner$ agents avoid exploitation by randomising between $H$ and $T$ to obtain a near-optimal NDR value (0) for this game.
    In contrast to other methods, $SQLearner$ agents have close to zero variance across runs. 
    }
    \label{fig:results_IMP}
\end{figure}

We train different learners to play the IMP game.
The optimal policy for an agent to avoid exploitation is to play $H$ or $T$ perfectly randomly and obtain an NDR of $0$.
Figure~\ref{fig:results_IMP} shows the results. 
$SQLearner$ agents learn to play optimally and obtain an NDR close to $0$. 
Interestingly, Selfish Learner and Lola-PG agents converge to an exploiter-exploited equilibrium where one agent consistently exploits the other agent. 
This asymmetric exploitation equilibrium is more pronounced for Selfish Learner agents than for Lola-PG agents.
As before, we observe that $SQLearner$ agents have close to zero variance across runs, unlike other methods where the variance in NDR across runs is significant. 

Appendix \ref{appendix:results:ish} shows the results for the ISH game. 

\subsection{Evolving Cooperation in Games with visual input using GameDistill followed by SQLoss}
\label{sec:results:visual-input-gamedistll-and-sqloss}

\subsubsection{The Coin Game: GameDistill}
{
% \setlength{\belowdisplayskip}{0pt} \setlength{\belowdisplayshortskip}{0pt}
% \setlength{\abovedisplayskip}{0pt} \setlength{\abovedisplayshortskip}{0pt}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/100d-feature-vec.png}
    \caption{
Representation of the clusters learned by $GameDistill$.
Each point is a t-SNE projection of the 100-dimensional feature vector output by the \ipdistill network for an input sequence of states.  
The figure on the left is colored based on actual rewards obtained by each agent (Red agent followed by Blue agent).
The figure on the right is colored based on clusters learned by $GameDistill$. 
$GameDistill$ correctly identifies two types of state sequences, one for cooperation (blue cluster) and the other for defection (red cluster). 
}
\label{fig:feature_vector_plots}%
\end{figure}
}

\begin{comment}
\begin{figure}[t]
    \centering
    % \begin{subfigure}[t]{0.4\linewidth}
    %     \includegraphics[width=\linewidth]{images/results__CoinGame__IPD_formulation.png}
    %     \caption{Average NDR}
    %     \label{fig:results_CoinGame_IPD_formulation}
    % \end{subfigure}\hfil%
    \begin{subfigure}[t]{\linewidth}
        \includegraphics[width=\linewidth]{images/CoinGame_results_corrected.png}
        \caption{
        Probability of an agent eating a coin of its color
        }
        \label{fig:results_CoinGame_probability_of_eating_coin}
    \end{subfigure}
    \caption{\label{fig:coingame_results}%
    Average NDR (a) and cooperation level (b) for learners trained in the Coin Game. 
    $SQLearner$ agents cooperate (eat only their own coins) to obtain near optimal NDR (-0.5) in the game. 
    }
\end{figure}
\end{comment}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.65\linewidth]{images/CoinGame_results_corrected.png}
    \caption{\label{fig:coingame_results}%
    Probability of an agent picking a coin of its color for learners trained in the Coin Game. 
    $SQLearner$ agents cooperate (pick only their own coins) to achieve a near optimal strategy in the game. 
    In contrast to Lola-PG, $SQLearner$ agents have close to zero variance across runs. 
    }
\end{figure}




To evaluate the clustering step in \ipdistill, we make two t-SNE~\cite{maaten2008visualizing} plots of the 100-dimensional feature vector extracted from the last layer of the \ipdistill network. 
The first plot colors each point (state sequence) by the rewards obtained by both agents in the sequence.
The second plot colors each point by the cluster label output by Agglomerative clustering.
Figure~\ref{fig:feature_vector_plots} shows the results. 
\ipdistill correctly learns two clusters, one for state sequences that represent cooperation and the other for state sequences that represent defection.
We also experiment with different values for feature vector dimensions and obtain similar clustering results with sufficient training. 
Once we have the clusters, we train oracle networks using the state sequences in each cluster.
To evaluate that the trained oracles represent a cooperation and a defection policy, we modify the Coin Game environment to contain only the Red agent.
We then play two variations of the game.
In the first variation, the Red agent is forced to play the action suggested by the first oracle. 
In this variation, we find that the Red agent picks only $8.4\%$ of Blue coins, indicating a high rate of cooperation. 
Therefore, the first oracle represents a cooperation policy. 
In the second variation, the Red agent is forced to play the action suggested by the second oracle. 
In this case, we find that the Red agent picks $99.4\%$ of Blue coins, indicating a high rate of defection. 
Hence, the second oracle represents a defection policy.
Therefore, the oracles learned by the Red agent using \ipdistill represent cooperation and defection policies. 

\subsubsection{The Coin Game: SQLoss}
Before playing the game, each $SQLearner$ agent uses \ipdistill to learn cooperation and defection oracles. 
During game-play, at each step, an agent follows either the action suggested by its cooperation oracle or the action suggested by its defection oracle. 
Further, each $SQLearner$ agent has an additional $SQLoss$ term.
We compare approaches using the degree of cooperation between agents, measured by the probability of an agent to pick the coin of its color~\cite{foerster2018learning}.  
Figure~\ref{fig:coingame_results} shows the results. 
The probability that an $SQLearner$ agent will pick the coin of its color is close to $1$. 
This high probability indicates that the other $SQLearner$ agent is cooperating with this agent and only picking coins of its color. 
In contrast, the probability that a Lola-PG agent will pick its own coin is much smaller, indicating higher rates of defection.
As expected, the probability of an agent picking its own coin is the smallest for selfish learners (SL). 
The probability value of $0.5$ indicates that a selfish learner is just as likely to pick the other agent's coin as it is to pick its own coin. 

\subsection{SQLearner: Exploitability and Adaptability}
Given that an agent does not have any prior information about the other agent, it is important that it evolves its strategy based on the strategy of its opponent. 
To evaluate an $SQLearner$ agent's ability to avoid exploitation by a selfish agent, we train one $SQLearner$ agent against an agent that always defects in the Coin Game. 
We find that the $SQLearner$ agent also learns to always defect.
This persistent defection is important since given that the other agent is selfish, the $SQLearner$ agent can do no better than also be selfish. 
To evaluate an $SQLearner$ agent's ability to exploit a cooperative agent, we train one $SQLearner$ agent with an agent that always cooperates in the Coin Game. 
In this case, we find that the $SQLearner$ agent learns to always defect.
This persistent defection is important since given that the other agent is cooperative, the $SQLearner$ agent obtains maximum reward by behaving selfishly. 
Hence, the $SQLearner$ agent is both resistant to exploitation and able to exploit, depending on the strategy of the other agent.

\begin{comment}
\begin{table}
    \centering
    \begin{tabular}{|c|c|c|c|}
        \hline
        \multicolumn{1}{|p{1.3cm}|}{\multirow{3}{*}{\parbox{1.3cm}{\centering\textbf{Color of Coin}}}} & \multirow{3}{*}{\parbox{1.3cm}{\centering\textbf{Max steps}}} & \multicolumn{2}{c|}{\textbf{Percentage of coins picked}}\\ \cline{3-4}
        & & \multicolumn{1}{m{1.7cm}|}{\centering\textbf{Defection Skill}} & \multicolumn{1}{m{1.7cm}|}{\centering\textbf{Cooperation Skill}}\\ \hline
        
        %% AAMAS submitted results
        % \multirow{2}{*}{Red} & Max 1 steps & 50.8\% & 47.5\% \\ \cline{2-4}
        % & Max 2 steps & 95.4\% & 95.6\% \\ \hline
        % \multirow{2}{*}{Blue} & Max 1 steps & 50.8\% & 11.3\% \\ \cline{2-4}
        % & Max 2 steps & 95.4\% & 17.8\% \\ \hline
        
        %%% 2nd set of results
        % \multirow{2}{*}{Red} & Max 1 steps & 12.6\% & 34.7\% \\ \cline{2-4}
        % & Max 2 steps & 22.5\% & 71.0\% \\ \hline
        % \multirow{2}{*}{Blue} & Max 1 steps & 36.6\% & 8.1\% \\ \cline{2-4}
        % & Max 2 steps & 83.4\% & 14.6\% \\ \hline

        %% Latest set of results where the Cooperation oracle eats Red and Defection oracle eats the Blue coins ONLY.
        \multirow{2}{*}{Red} & 1 steps & 12.7\% & 46.7\% \\ \cline{2-4}
        & 2 steps & 22.4\% & 95.8\% \\ \hline
        \multirow{2}{*}{Blue} & 1 steps & 48.4\% & 4.7\% \\ \cline{2-4}
        & 2 steps & 99.4\% & 8.4\% \\ \hline

    \end{tabular}
    \caption{For Coin game. Percentage of coins picked by the \textit{Red} agent when the actions are predicted by the oracle trained from the events obtained by \ipdistill.}
    \label{tab:action_prediction_performance}
\end{table}
\end{comment}

\begin{comment}

\begin{table}
    \centering
    \begin{tabular}{|c|p{2cm}|p{2cm}|}
        \hline
        \multirow{3}{*}{\textbf{Oracle}}  & \multicolumn{2}{c|}{\textbf{Consumed coins}}\\
        & \multicolumn{2}{c|}{\textbf{(as a percentage of appeared coins)}} \\
        \cline{2-3}
        & {\centering\textbf{Red}} & {\centering\textbf{Blue}}\\ \hline
        %% Latest set of results where the Cooperation oracle eats Red and Defection oracle eats the Blue coins ONLY.
        Oracle 1 & 22.4\% & 99.4\% \\ \hline
        Oracle 2 & 95.8\% & 08.4\% \\ \hline
    \end{tabular}
    \caption{
    Examining the behavior of learned oracles for the Red agent in the Coin Game (when the environment does not contain the Blue agent).
    The Red agent eats almost all of the Blue coins when following oracle 1. 
    This indicates that oracle 1 represents the defection oracle. 
    Similarly, oracle 2 represents the cooperation oracle. 
    }
    \label{tab:action_prediction_performance}
\end{table}

\end{comment}


==> related_work.tex <==
\section{Related Work}
\label{sec:related_work}
Social dilemma problems brings out the conflict between an individual and the society and
Prisoner's dilemma \cite{Rapoport1974} has been used to highlight this core conflict. In-spite of several examples of cooperation in nature at various scales, from microscopic \cite{Szathmary1995}, to species level \cite{Heinsohn1995ComplexCS} including humans\cite{kleiman2016coordinate}, still greedy behavior leads to tragedy of the commons \cite{psychology_social_dilemmas}

There has been a large body of work which had looked at the mechanism of emergence of cooperation through reciprocal behaviour and indirect reciprocity \cite{reciprocal1971},\cite{reciprocal1984},\cite{reciprocal1992},\cite{reciprocal1993},\cite{in_reciprocal1998}, though variants of reinforcement using aspiration \cite{reinforce_variant}, attitude\cite{NonRL_attitude} or using multi-agent reinforcement learning \cite{Sandholm1996MultiagentRL,Wunder:2010}, under specific conditions \cite{R_plus_S_g_2P}, using different learning rates \cite{deCote:2006} similar to WoLF \cite{WOLF2002} as well as using embedded emotion \cite{Emotional_Multiagent}.

But with the advent of deep reinforcement learning~\cite{Mnih:2013,Mnih:2015}, recent work on social dilemma problem have taken a rather hands off approach with the idea of letting agents figure out strategies, all by themselves. In the paper~\cite{Leibo:2017} the authors have setup the problem of social dilemma in deep reinforcement learning framework and have analyzed the outcome of the 2d Fruit gathering game as general sum matrix games, where by varying the abundance of resources and cost of conflict, they generate varying degrees of cooperation. In~\cite{Hughes:2018}, they define an intrinsic reward called inequality aversion which tries to reduce difference in rewards among the agents by having aversion to both advantageous(guilt) and disadvantageous(unfairness) inequity. This handcrafting of loss with mutual fairness leads to better cooperation but also makes the agent vulnerable to exploitation. The authors in~\cite{foerster2018learning} propose LOLA, where they achieve high degree of cooperation in their Coin game and Iterative Prisoner's Dilemma. They do this by having access to the opponent policy parameters and gradients. This is equivalent to getting access to opponent's brain and devising strategy with the knowledge of how they are about to play. In a more recent paper~\cite{Wang:2019}, \citeauthor{Wang:2019} proposes an evolutionary based deep reinforcement learning setup to evolve cooperation. They define an intrinsic reward which is based on a feature, generated from agent's past and expected future rewards and this feature is shared with other agents. They then use evolution to maximise the sum of rewards among the agents which leads to achieving cooperation. This is an indirect method of maximizing the sum of rewards for the society which would lead to cooperation.
Another paper \cite{Wang:2018} proposed a method, where they start with two policies, cooperation($\pi_C$) and defection ($\pi_D$). With these they generate several intermediate policies with varying degrees of ($\pi_C$) and ($\pi_D$) and then during gameplay each agent tries to predict the degree of cooperation by its opponent and chooses a matching policy of same degree of cooperation. This is an indirect way of hard coding a strategy like Tit-For-Tat because both agent try to mimic the opponent's perceived policy rather than playing to maximize their respective rewards. In contrast to these methods we try to develop cooperation using a status-quo loss, without inducing any strategy bias towards cooperation.

In \cite{consequentialist18}, \citeauthor{consequentialist18} takes the direction of having predefined policies of cooperation($\pi_C$) and defection ($\pi_D$) and have built in a handcrafted mechanism of playing multiple rollouts of actions $CC$ and $CD$ to figure out the payoffs for these strategies. Subsequently, they use a rule based mechanism to choose between cooperation($\pi_C$) and defection ($\pi_D$) policies. Their idea of having existing policies of ($\pi_C$) and ($\pi_D$) is similar to our idea of learning skills of cooperation or defection. However, we try to discover these policies using a self-supervised clustering method while playing the game in a random manner (i.e. random action policy). 

% \citet{kleiman2016coordinate} studied the emergence of cooperation and defection for humans and compare it results from agents learnt using reinforcement-learning.
